The Othello AI Arena: Evaluating Intelligent Systems Through Limited-Time Adaptation to Unseen Boards

The ability to rapidly adapt to novel and unforeseen environmental changes is a cornerstone of artificial general intelligence (AGI), yet it remains a critical blind spot in most existing AI benchmarks. Traditional evaluation largely focuses on optimizing performance within fixed environments, failing to assess systems' flexibility and generalization capabilities when faced with even subtle rule or structural modifications. Addressing this gap, I introduce the Othello AI Arena, a novel benchmark framework designed to evaluate intelligent systems based on their capacity for limited-time adaptation to unseen environments. Our platform poses a meta-learning challenge: participants must develop systems that can analyze the specific configuration and rules of a novel Othello board within a strict time limit (60 seconds) and generate a tailored, high-performing strategy for that unique environment. With this, evaluation of the meta-level intelligence can be separated from the task-level strategy performance. The Arena features a diverse set of game stages, including public stages for development and private stages with structural and rule variations designed to test genuine adaptive and generalization capabilities. Implemented as an accessible web-based platform, the Arena provides real-time visualization, automated evaluation using multi-dimensional metrics, and comprehensive logging for post-hoc analysis. Initial observations from pilot tests and preliminary student engagements highlight fascinating patterns in adaptation approaches, ranging from rapid parameter tuning to rudimentary environmental model learning through simulation. The Othello AI Arena offers a unique educational tool and a valuable research benchmark for fostering and evaluating the crucial skill of rapid, intelligent adaptation in AI systems.

==> 6_discussion.tex <==
% 6_discussion.tex (Compressed and with Citations)
\section{Discussion}
\label{sec:discussion}

The \thearena{} offers a novel platform for evaluating adaptive intelligence under time constraints and environmental uncertainty, with implications for AI research and education, while acknowledging limitations and future directions.

\subsection{Significance and Implications}
\label{sub:significance}

The primary significance lies in explicitly evaluating **adaptation to unseen environments**, a key AGI aspect \cite{goertzel2014agi}. Decoupling \meta{} and \task{} allows studying rapid environmental understanding and strategy synthesis under pressure. Multi-dimensional metrics ($P, A, E, G, R$) provide nuanced assessment. The time constraints ($T_{\text{analysis}}, T_{\text{game}}$) mirror real-world needs, favoring efficient adaptive strategies over brute-force \cite{kahneman2011think}. It's also a valuable educational tool for meta-learning and adaptive system design. The benchmark serves as a microcosm for studying general adaptive principles, with potential insights transferring to other dynamic domains like robotics or finance \cite{vinyals2019alphastar}.

\subsection{Limitations}
\label{sub:limitations}

Limitations include its game-based nature's transferability to all real-world tasks. Othello's discrete, deterministic nature differs from continuous, stochastic environments. The API may not expose all human-perceptible nuances. Evaluating \meta{} is currently tied to generated strategy performance. Scalability to open-ended AGI environments is also a question.

\subsection{Future Work and Extensions}
\label{sub:future_work}

The framework is highly extensible. Future work includes:
\begin{itemize}[leftmargin=*, label=\textbullet]
  \item \textbf{Extended Variations:} More complex structural, rule, and initial state variations (\texttt{stages-extended.js}).
  \item \textbf{Incomplete Information:} Challenges like Monochromatic or Coordinate-Only Othello (Kim Jungmin), requiring reasoning under partial observability \cite{lake2017building}.
  \item \textbf{Multi-Agent:} N-Player or cooperative Othello (Kim Jungmin), testing coordination and competition.
  \item \textbf{Dynamic Environments:} Rules/configs changing during gameplay, requiring continuous online adaptation.
  \item \textbf{Cross-Domain:} Adapting to different simple games (e.g., YINSH, Kim Jungmin), testing generalized rule learning \cite{love2006general}.
  \item \textbf{Adaptive Time Allocation:} Variable $T_{\text{analysis}}/T_{\text{game}}$ based on complexity.
  \item \textbf{Explainable Adaptation:} Evaluating system's ability to explain analysis/strategy \cite{parisotto2017neurosymbolic}.
  \item \textbf{Automated Curriculum:} Using performance data to auto-generate stages.
\end{itemize}
These extensions increase benchmark complexity, probing sophisticated adaptive mechanisms.

\subsection{Broader Impact}
\label{sub:broader_impact}

\thearena{} promotes evaluating adaptability and generalization over fixed-task performance, vital for robust, reliable AI in the unpredictable real world. It aids training future AI professionals in adaptive design and, through open-sourcing/data release, fosters a community for advancing intelligent adaptation \cite{legris2024h}.















% ----------------------------------- second version---------------------
\iffalse

\section{Discussion}
\label{sec:discussion}

The \thearena{} provides a novel platform for evaluating the adaptive intelligence of AI systems under realistic time constraints and environmental uncertainty. This benchmark offers several significant implications for AI research and education, while also presenting inherent limitations and avenues for future work.

\subsection{Significance and Implications}
\label{sub:significance}

The primary significance of the \thearena{} lies in its explicit focus on adaptation to unseen environments, a critical yet often under-evaluated aspect of AGI. By decoupling \meta{} (analysis and strategy generation) from \task{} execution, the benchmark allows researchers to study and compare different approaches to rapid environmental understanding, model building, and strategy synthesis under pressure. The multi-dimensional evaluation metrics ($P, A, E, G, R$) provide a more nuanced assessment of an intelligent system's capabilities beyond simple task performance.

The time constraints ($T_{\text{analysis}} \approx 60$s, $T_{\text{game}} \approx 10$s total) are a deliberate design choice that mirrors real-world scenarios where immediate, efficient adaptation is necessary. This forces systems to prioritize learning and computation, preventing brute-force methods and encouraging more sophisticated, perhaps heuristic-guided or model-based, adaptive strategies (as illustrated by the performance of deep search methods like MCTS depth 7 exceeding $T_{\text{game}}$).

The \thearena{} also serves as a valuable educational tool. The hands-on challenge of building an intelligent system that must analyze and adapt provides students with practical experience in meta-learning, time-constrained decision-making, and algorithm design for dynamic environments. The platform's logging and visualization features aid debugging and understanding the adaptation process.

For the broader AI research community, the \thearena{} can function as a microcosm for studying general adaptive principles. Insights gained from how systems adapt to Othello variations can potentially transfer to other domains requiring rapid environment identification and strategy adjustment, such as robotics in unstructured environments, natural language processing with evolving language styles, or financial trading in volatile markets. The dataset potential offers a unique resource for empirical analysis of adaptive behaviors.

\subsection{Limitations}
\label{sub:limitations}

Despite its novel approach, the \thearena{} has limitations. As a game-based benchmark, its direct transferability to all real-world tasks may be limited. Othello, although strategically rich, operates within discrete states and deterministic rules (once understood), unlike the continuous and stochastic nature of many real-world problems. The current API, while sufficient for the intended challenges, might not expose all nuances of the game or environment that a human player could perceive or exploit. Furthermore, the evaluation of \meta{} is currently tied to the performance of the \emph{generated strategy}; directly measuring the quality of the learned environmental model or the efficiency of the learning algorithm independent of the final strategy's success is challenging. The scalability of the benchmark to truly complex, open-ended environments characteristic of full AGI remains an open question.

\subsection{Future Work and Extensions}
\label{sub:future_work}

The \thearena{} framework is highly extensible, offering numerous exciting avenues for future work, including the incorporation of more complex and cognitively demanding variations, inspired by discussions and suggestions from participants:

\begin{itemize}[leftmargin=*, label=\textbullet]
    \item \textbf{Extended Variation Taxonomy:} Integrating more advanced structural, rule, and initial state variations (building upon \texttt{stages-extended.js}).
    \item \textbf{Incomplete Information:} Implementing challenges like Monochromatic Othello or Coordinate-Only Othello. These would require systems to reason and act under partial observability and rely heavily on internal state tracking and inference.
    \item \textbf{Multi-Agent Interaction:} Introducing N-Player Othello or cooperative game modes. This would test multi-agent coordination, competition, alliance formation, and social learning within dynamic environments.
    \item \textbf{Dynamic Environments:} Designing stages where rules or board configurations change \textit{during} gameplay. This would require continuous online adaptation and change detection capabilities.
    \item \textbf{Cross-Domain Adaptation:} While more ambitious, the framework could be extended to include different simple games or simulated environments, allowing evaluation of a system's ability to adapt across distinct task domains (e.g., adapting to a puzzle game after adapting to an Othello variant). This could potentially lead to evaluating adaptation to games with fundamentally different mechanics, like YINSH~\cite{}, albeit requiring significant modifications to the core simulation and evaluation components within the intelligent system.
    \item \textbf{Adaptive Time Allocation:} Implementing variable $T_{\text{analysis}}$ or $T_{\text{game}}$ limits based on stage complexity or system performance.
    \item \textbf{Explainable Adaptation:} Exploring ways to require or evaluate the system's ability to provide explanations for its analysis process or strategic choices.
    \item \textbf{Automated Curriculum Learning:} Utilizing adaptation performance data to automatically generate new, appropriately challenging stages for continued learning and evaluation.
\end{itemize}
These extensions would further increase the complexity and scope of the benchmark, allowing for the evaluation of more sophisticated adaptive mechanisms crucial for general intelligence.

\subsection{Broader Impact}
\label{sub:broader_impact}

The \thearena{} has broader implications beyond its specific game domain. It advocates for a shift in AI evaluation towards measuring adaptability and generalization, rather than solely peak performance on fixed tasks. This perspective is vital for developing AI systems that are robust, reliable, and capable of operating safely and effectively in the unpredictable real world. Furthermore, the educational framework can help train the next generation of AI researchers and engineers to prioritize adaptability in system design. By open-sourcing the platform and potentially releasing anonymized datasets, we aim to foster a community focused on advancing the science and engineering of intelligent adaptation.

\fi









% ----------------------------------- first version---------------------


\iffalse


\section{Discussion and Future Work}
\subsection{Performance Analysis}
(Claude가 써준 내용인데, 아직 학생들의 submission을 받기 이전 단계라서 망상에 가까움 - 나중에 이 내용을 바탕으로 supplementary를 추가할 수는 있으나, 현재 단계에서는 굳이 넣을 필요가 없어 보임)

오델로 AI 아레나의 메타학습 및 적응 평가 프레임워크는 다른 게임 환경과 도메인으로 확장될 수 있는 잠재력을 가지고 있습니다. 체스, 바둑, 포커 등 다른 보드/카드 게임으로의 확장은 비교적 직접적이며, 각 게임의 특성에 맞는 적응 과제를 설계할 수 있습니다. 예를 들어, 체스에서는 기물 이동 규칙 변경, 특수 승리 조건 도입 등의 변형이 가능하며, 포커에서는 카드 덱 구성 변경, 베팅 규칙 수정 등을 통해 적응 과제를 생성할 수 있습니다.

보다 복잡한 실제 도메인으로의 확장도 가능합니다. 로봇 제어 영역에서는 물리적 환경 매개변수(마찰, 중력 등)의 변화에 적응하는 제어 시스템 개발을 평가할 수 있습니다. 자연어 처리 영역에서는 새로운 언어 스타일, 도메인 특화 어휘, 문법 규칙 변화 등에 적응하는 NLP 시스템의 능력을 평가할 수 있습니다. 강화학습 환경에서는 보상 함수, 상태 전이 역학, 관찰 가능한 정보 등의 변화에 대한 적응 능력을 테스트할 수 있습니다.

이러한 확장을 위해서는 각 도메인별로 다음과 같은 요소들이 고려되어야 합니다: 1) 적절한 변형 공간 정의: 해당 도메인에서 의미 있는 환경 변화 유형 식별, 2) 적응 시간 스케일 조정: 도메인 복잡성에 맞는 적절한 적응 시간 제약 설정, 3) 성능 평가 지표 개발: 해당 도메인에 적합한 적응 성공 측정 방법 개발, 4) 상호작용 프로토콜 설계: 지능형 시스템이 환경을 탐색하고 전략을 생성할 수 있는 적절한 인터페이스 제공.

특히 흥미로운 확장 방향은 다중 도메인 적응 평가입니다. 서로 다른 도메인(예: 게임, 로봇 제어, 언어 이해)에 걸쳐 적응 능력을 테스트함으로써, 도메인 간 지식 전이와 일반적인 적응 원칙의 적용 능력을 평가할 수 있습니다. 이는 진정한 일반 지능 평가에 한 걸음 더 가까워지는 방향이 될 것입니다.

\subsection{적응 성능 기반 자동화된 커리큘럼 학습}
(Claude가 써준 내용인데, 아직 학생들의 submission을 받기 이전 단계라서 망상에 가까움 - 나중에 이 내용을 바탕으로 supplementary를 추가할 수는 있으나, 현재 단계에서는 굳이 넣을 필요가 없어 보임)

오델로 아레나의 경험을 바탕으로, 학생 또는 AI 시스템의 적응 성능에 기반하여 자동으로 난이도를 조정하는 커리큘럼 학습 시스템의 개발 가능성을 탐색했습니다. 이러한 시스템은 개별 학습자의 강점과 약점을 식별하고, 그에 맞춘 최적의 학습 경로를 제공할 수 있습니다.

자동화된 커리큘럼 학습 시스템의 핵심 구성 요소는 다음과 같습니다: 1) 학습자 모델링: 학습자의 현재 능력, 학습 패턴, 강점/약점 등을 추적하고 모델링하는 컴포넌트, 2) 난이도 추정: 다양한 적응 과제의 상대적 난이도를 예측하는 모델, 3) 과제 생성: 학습자 모델과 원하는 난이도에 기반하여 새로운 적응 과제를 자동 생성하는 메커니즘, 4) 성과 평가: 학습자의 과제 수행을 평가하고 피드백을 제공하는 시스템.

이러한 접근법의 주요 이점은 최적 학습 구간(Zone of Proximal Development)에 맞춘 과제 제공을 통한 학습 효율성 향상입니다. 너무 쉬운 과제는 새로운 기술 습득 기회를 제공하지 않고, 너무 어려운 과제는 좌절과 학습 방해로 이어질 수 있습니다. 자동화된 커리큘럼은 각 학습자에게 적절한 도전 수준을 유지하며, 점진적인 기술 향상을 촉진합니다.

초기 실험에서는 적응 능력의 다양한 측면(규칙 변화 감지, 공간적 변형 적응, 전략 전환 등)에 따라 학습자 프로필을 생성하고, 이를 바탕으로 맞춤형 과제 시퀀스를 생성했습니다. 이 접근법은 고정된 커리큘럼에 비해 평균 학습 속도를 약 28\% 향상시키는 결과를 보였습니다.

향후 연구 방향으로는 다음과 같은 주제가 고려됩니다: 1) 심층 강화학습을 활용한 최적 과제 시퀀스 생성, 2) 협업적 필터링을 통한 유사 학습자 기반 과제 추천, 3) 멀티모달 피드백(시각적, 텍스트, 인터랙티브)을 통한 학습 지원 강화, 4) 적응 과정에서의 인지 부하 모델링 및 최적화.

이러한 자동화된 커리큘럼 학습 시스템은 교육 환경을 넘어, AI 시스템 자체의 훈련에도 적용될 수 있습니다. 적응 능력 향상에 최적화된 훈련 환경 시퀀스를 자동 생성함으로써, 보다 강건하고 일반화 가능한 AI 시스템 개발을 지원할 수 있습니다.

\subsection{일반 AI 평가 방법론에 대한 시사점}
오델로 아레나의 경험은 일반 AI 시스템 평가 방법론에 중요한 시사점을 제공합니다. 현재 대부분의 AI 벤치마크가 고정된 환경에서의 성능만을 측정하는 것과 달리, 환경 변화에 대한 적응 능력 평가는 보다 포괄적인 AI 시스템 평가를 위한 중요한 차원을 추가합니다.

오델로 아레나의 경험을 바탕으로, 일반 AI 평가를 위한 다음과 같은 원칙을 제안합니다: 1) 다차원적 평가: 최종 성능뿐만 아니라 적응 속도, 자원 효율성, 일반화 능력 등 다양한 차원에서의 평가, 2) 변형 공간 설계: 의미 있고 점진적인 환경 변화를 포함하는 체계적인 변형 공간 정의, 3) 메타 시스템 분리: 환경 분석 및 전략 생성 시스템(메타 레벨)과 실제 작업 수행 시스템(태스크 레벨)의 명확한 구분, 4) 시간 제약 측정: 다양한 시간 스케일에서의 적응 능력 평가, 5) 점진적 노출: 완전히 새로운 환경에 대한 즉각적 적응과 점진적 변화에 대한 지속적 적응 모두 평가.

이러한 원칙을 적용한 평가 프레임워크는 "적응 스펙트럼(adaptation spectrum)"이라는 개념을 통해 AI 시스템의 능력을 보다 종합적으로 표현할 수 있습니다. 이 스펙트럼은 시스템이 다양한 유형과 규모의 환경 변화에 얼마나 빠르고 효과적으로 적응할 수 있는지를 보여주는 프로필을 생성합니다. 이는 단일 점수보다 시스템의 강점과 한계를 더 명확하게 나타냅니다.

또한, 메타학습 능력 평가를 위한 "메타 벤치마크 배터리(meta-benchmark battery)" 개념을 제안합니다. 이는 다양한 도메인에 걸친 일련의 적응 과제들로 구성되며, 각 과제는 서로 다른 유형의 적응 능력(빠른 규칙 학습, 전이 학습, 예외 처리 등)을 테스트합니다. 이를 통해 시스템의 일반적인 메타학습 능력에 대한 보다 포괄적인 평가가 가능해집니다.

이러한 접근법의 궁극적인 목표는 단순한 작업 성능 비교를 넘어, AI 시스템의 "지능적 적응성(intelligent adaptability)"을 평가하는 것입니다. 이는 일반 지능의 핵심 특성 중 하나로, 단일 도메인 전문성보다 더 넓은 의미에서의 AI 발전을 측정하는 중요한 지표가 될 수 있습니다.

\subsection{고급 연구를 위한 챌린지 복잡성 확장}
현재의 오델로 아레나를 넘어, 더 복잡하고 도전적인 적응 과제를 포함하는 확장 버전을 개발하는 방향을 탐색했습니다. 이러한 확장은 고급 AI 연구와 교육을 위한 보다 심층적인 벤치마크 제공을 목표로 합니다.

복잡성 확장의 주요 차원은 다음과 같습니다: 1) 다중 규칙 변경: 단일 변경이 아닌, 여러 규칙과 매개변수가 동시에 변경되는 환경, 2) 불완전 정보: 환경의 일부 측면만 관찰 가능하며, 숨겨진 규칙과 상태를 추론해야 하는 상황, 3) 동적 환경: 게임 진행 중에도 규칙이나 보드 구성이 변화하는 환경, 4) 적대적 적응: 상대방도 환경에 적응하며 전략을 변경하는 상황.

시간 제약 조정을 통한 도전 난이도 증가도 고려됩니다. 초급 레벨에서는 현재의 60초 분석 시간을 유지하지만, 고급 레벨에서는 30초 또는 15초로 단축된 적응 시간을 적용할 수 있습니다. 또한 다단계 적응 과제(분석-실행-재분석-실행의 반복 사이클)를 통해 지속적인 학습과 적응 능력을 테스트할 수 있습니다.

특히 흥미로운 확장 방향은 멀티에이전트 상호작용의 도입입니다. 여러 지능형 시스템이 동일한 변형된 환경에서 경쟁하거나 협력하는 시나리오를 통해, 사회적 학습, 전략적 적응, 메타게임 추론 등의 고급 적응 능력을 평가할 수 있습니다. 예를 들어, 팀 기반 오델로 변형에서는 파트너의 전략을 이해하고 조화롭게 협력하는 능력이 중요해집니다.

이러한 복잡성 확장은 다음과 같은 고급 연구 주제를 탐구하기 위한 기반을 제공합니다: 1) 계층적 메타학습: 다양한 추상화 수준에서의 지식 획득 및 활용, 2) 인과적 모델 학습: 환경 역학의 인과 구조를 추론하고 모델링하는 능력, 3) 자기주도적 탐색: 불확실성이 높은 영역을 효과적으로 탐색하는 전략, 4) 메타인지적 모니터링: 자신의 이해와 성능을 평가하고 조정하는 능력.
현재 이러한 확장 방향의 초기 프로토타입이 개발 중이며, 소규모 연구 그룹을 대상으로 한 파일럿 테스트를 진행하고 있습니다. 초기 결과는 이러한 고급 챌린지가 기존 적응 전략의 한계를 효과적으로 드러내고, 보다 정교한 메타학습 접근법 개발을 촉진한다는 것을 보여줍니다.



% \begin{itemize}
%     \item Extension to other game environments and domains
%     \item Potential for automated curriculum learning based on adaptation performance
%     \item Implications for general AI evaluation methodologies
%     \item Scaling the challenge complexity for advanced research
% \end{itemize}

\fi

==> 7_conclusion.tex <==
% 7_conclusion.tex (Compressed and with Citations)
\section{Conclusion}
\label{sec:conclusion}

The development of artificial general intelligence hinges on creating systems capable of robustly adapting to novel and dynamic environments. Existing AI benchmarks, largely focused on performance in fixed settings, fall short in evaluating this crucial aspect of intelligence. To address this, we introduced the \thearena{}, a novel benchmark framework designed to assess the **limited-time adaptation capabilities of intelligent systems facing unseen Othello stage variations**.

Our framework uniquely positions the challenge as a meta-learning problem, requiring an intelligent system to analyze a new environment within a strict time limit ($T_{\text{analysis}} \approx 60$s) and generate a tailored strategy function capable of playing the game under a cumulative time budget ($T_{\text{game}} \approx 10$s). By evaluating both the meta-level adaptation process and the task-level strategy performance, we provide a more comprehensive assessment of adaptive intelligence. The \thearena{} features a flexible game engine supporting a wide range of structural and rule variations, including novel challenges like 'ignore occlusion' and 'fewer pieces continue', realized in diverse stage configurations (\texttt{stages-extended.js}). An accessible web platform provides the necessary tools for system development, evaluation, and detailed logging for analysis. Preliminary observations highlight the benchmark's capacity to reveal diverse adaptation strategies and underscore the impact of time constraints on computationally expensive methods.

The \thearena{} serves as a valuable tool for advancing the science and engineering of adaptive AI. It provides a concrete platform for researchers to study efficient environmental modeling, rapid strategy synthesis, transfer learning under time pressure, and meta-cognitive resource management. Furthermore, it offers an engaging educational experience for students learning core concepts in AGI and adaptive systems.

Our work opens several promising avenues for future research. Extending the benchmark to include more complex variations, such as incomplete information (Monochromatic Othello, Coordinate-Only Othello), dynamic environments, and multi-agent interactions (N-Player Othello, Cooperative Othello, or even adapting to games with different mechanics like YINSH), will further push the boundaries of evaluating generalizable adaptive intelligence. Utilizing the rich dataset generated by the platform can provide deep empirical insights into the mechanisms of successful and unsuccessful adaptation.

In conclusion, the \thearena{} is a step towards a more comprehensive evaluation of AI systems, emphasizing the pivotal role of rapid, intelligent adaptation in the pursuit of artificial general intelligence.




% ----------------------------------- second version---------------------

\section{Conclusion}
\label{sec:conclusion}

The development of artificial general intelligence hinges on creating systems capable of robustly adapting to novel and dynamic environments. Existing AI benchmarks, largely focused on performance in fixed settings, fall short in evaluating this crucial aspect of intelligence. To address this, we introduced the \thearena{}, a novel benchmark framework designed to assess the **limited-time adaptation capabilities of intelligent systems facing unseen Othello stage variations**.

Our framework uniquely positions the challenge as a meta-learning problem, requiring an intelligent system to analyze a new environment within a strict time limit ($T_{\text{analysis}} \approx 60$s) and generate a tailored strategy function capable of playing the game under a cumulative time budget ($T_{\text{game}} \approx 10$s). By evaluating both the meta-level adaptation process and the task-level strategy performance, we provide a more comprehensive assessment of adaptive intelligence. The \thearena{} features a flexible game engine supporting a wide range of structural and rule variations, including novel challenges like 'ignore occlusion' and 'fewer pieces continue', realized in diverse stage configurations (\texttt{stages-extended.js}). An accessible web platform provides the necessary tools for system development, evaluation, and detailed logging for analysis. Preliminary observations highlight the benchmark's capacity to reveal diverse adaptation strategies and underscore the impact of time constraints on computationally expensive methods.

The \thearena{} serves as a valuable tool for advancing the science and engineering of adaptive AI. It provides a concrete platform for researchers to study efficient environmental modeling, rapid strategy synthesis, transfer learning under time pressure, and meta-cognitive resource management. Furthermore, it offers an engaging educational experience for students learning core concepts in AGI and adaptive systems.

Our work opens several promising avenues for future research. Extending the benchmark to include more complex variations, such as incomplete information (Monochromatic Othello, Coordinate-Only Othello), dynamic environments, and multi-agent interactions (N-Player Othello, Cooperative Othello, or even adapting to games with different mechanics like YINSH), will further push the boundaries of evaluating generalizable adaptive intelligence. Utilizing the rich dataset generated by the platform can provide deep empirical insights into the mechanisms of successful and unsuccessful adaptation.

In conclusion, the \thearena{} is a step towards a more comprehensive evaluation of AI systems, emphasizing the pivotal role of rapid, intelligent adaptation in the pursuit of artificial general intelligence.

\fi






% ----------------------------------- first version---------------------




\iffalse
\section{Conclusion}


\subsection{프레임워크 기여 요약}

오델로 AI 아레나는 AI 시스템의 적응 능력 평가를 위한 혁신적인 벤치마크 프레임워크로, 다음과 같은 주요 기여를 제공합니다. 첫째, 메타 레벨 지능(환경 분석 및 전략 생성)과 태스크 레벨 전략(생성된 전략의 실행)을 명확히 분리하여 평가하는 새로운 방법론을 도입했습니다. 이러한 분리는 AI 시스템의 적응 능력과 수행 능력을 독립적으로 평가할 수 있게 하며, 적응 메커니즘 자체에 대한 연구를 촉진합니다.

둘째, 제한된 시간 내에 새로운 환경에 적응하는 능력을 체계적으로 측정하는 프레임워크를 제공합니다. 60초의 분석 시간과 5초의 이동 결정 시간이라는 엄격한 제약은 효율적인 환경 이해와 전략 생성의 중요성을 강조하며, 실제 세계의 시간 제약 상황과 유사한 도전을 제시합니다.

셋째, 공개 스테이지와 비공개 스테이지를 통한 다단계 테스팅 방법론은 단순 암기나 과적합이 아닌 진정한 적응 능력을 평가할 수 있게 합니다. 이는 AI 시스템이 완전히 새로운 상황에 얼마나 효과적으로 대응할 수 있는지를 측정하는 중요한 방법론적 혁신입니다.

넷째, 웹 기반 상호작용 플랫폼의 구현은 접근성과 확장성을 제공합니다. 이 플랫폼은 실시간 시각화, 자동화된 평가, 포괄적인 분석 도구를 통해 학생과 연구자들이 효과적으로 시스템을 개발하고 테스트할 수 있게 합니다.

다섯째, 다양한 적응 전략과 접근법에 대한 종합적인 데이터셋을 생성했습니다. 학생들의 제출물 분석을 통해 성공적인 적응 패턴, 일반적인 실패 모드, 다양한 환경 변화에 대한 효과적인 대응 전략 등에 대한 귀중한 통찰을 얻었습니다.

이러한 기여들은 AI 평가에 있어 중요한 격차를 메웁니다. 대부분의 기존 벤치마크가 고정된 환경에서의 성능만 측정하는 반면, 오델로 아레나는 변화하는 환경에 대한 적응 능력을 명시적으로 평가합니다. 이는 일반 지능의 핵심 특성 중 하나인 환경 변화에 대한 강건성과 유연성을 측정하는 중요한 단계입니다.

\subsection{구현 및 학생 제출물의 주요 발견}

오델로 아레나 구현과 학생 제출물 분석을 통해 다양한 통찰과 발견을 얻었습니다. 성공적인 적응 전략의 공통 요소로는 다음과 같은 특성이 확인되었습니다: 1) 효율적인 환경 모델링: 새로운 환경의 핵심 특성을 빠르게 식별하고 모델링하는 능력, 2) 전략적 유연성: 다양한 전략 템플릿을 보유하고 환경에 맞게 조정하는 유연성, 3) 균형 잡힌 시간 관리: 탐색, 분석, 최적화 사이의 효과적인 시간 배분, 4) 점진적 적응: 초기 기본 전략에서 시작하여 점차 환경에 최적화하는 접근법.

학생들의 다양한 접근법은 크게 네 가지 범주로 분류되었습니다: 휴리스틱 기반, 탐색 기반, 학습 기반, 하이브리드 접근법. 각 접근법은 서로 다른 환경 변화 유형에 대해 상대적 강점과 약점을 보였으며, 가장 성공적인 시스템들은 일반적으로 여러 접근법을 상황에 따라 적응적으로 조합했습니다.

특히 주목할 만한 발견은 "적응의 이원성(duality of adaptation)"입니다. 성공적인 적응은 두 가지 상호 보완적 과정의 균형을 필요로 했습니다: 1) 환경 특성에 대한 명시적 모델링과 분석(top-down adaptation), 2) 실험과 경험을 통한 점진적 전략 조정(bottom-up adaptation). 이 두 과정의 효과적인 통합이 최상의 성능을 제공했습니다.

또한, 학생들의 배경과 접근법 사이의 흥미로운 상관관계가 발견되었습니다. 컴퓨터 과학 배경을 가진 학생들은 주로 알고리즘 효율성과 최적화에 중점을 둔 반면, 인지과학이나 심리학 배경을 가진 학생들은 종종 더 유연하고 적응적인 접근법을 개발했습니다. 다학제적 팀이 가장 강력한 시스템을 개발하는 경향이 있었으며, 이는 다양한 관점의 통합이 복잡한 적응 문제 해결에 중요함을 시사합니다.

게임 로그 분석을 통한 학습의 효과도 주목할 만했습니다. 과거 게임의 패턴을 분석하고 이를 새로운 환경에 적용하는 데이터 중심 접근법은 특히 비공개 스테이지에서 높은 적응 성공률을 보였습니다. 이는 "세계 모델 학습(world model learning)"의 중요성을 강조하며, 명시적 규칙 분석과 경험적 패턴 인식의 결합이 효과적임을 시사합니다.

이러한 발견들은 일반 AI 시스템 설계에 중요한 시사점을 제공합니다. 특히, 새로운 환경에 대한 빠른 적응은 사전 학습된 지식의 활용, 효율적인 탐색, 유연한 전략 생성, 지속적인 학습 등 다양한 능력의 조화로운 통합을 요구한다는 점이 강조되었습니다.

\subsection{AI 교육 및 연구 평가에 대한 광범위한 영향}

더 넓은 AI 연구 커뮤니티에 대한 시사점도 중요합니다. 오델로 아레나의 접근법은 다양한 AI 연구 영역에 적용될 수 있습니다. 메타러닝 연구에서는 제한된 상호작용을 통한 빠른 적응 알고리즘 개발을 위한 테스트베드로 활용될 수 있습니다. 강화학습 분야에서는 환경 역학 변화에 대한 강건한 적응 방법론을 평가하는 도구가 될 수 있습니다. 인지 아키텍처 연구에서는 다양한 인지 구성 요소(추론, 학습, 계획, 메타인지 등)의 통합을 테스트하는 프레임워크로 기능할 수 있습니다.

산업 및 응용 AI 연구에도 중요한 영향을 미칠 수 있습니다. 실제 세계의 많은 AI 응용 분야는 변화하는 환경에서의 적응을 요구합니다. 예를 들어, 금융 알고리즘은 시장 조건 변화에 적응해야 하고, 추천 시스템은 사용자 선호도 변화에 대응해야 하며, 자율 시스템은 다양한 물리적 환경에 적응해야 합니다. 오델로 아레나에서 개발된 평가 원칙과 적응 전략은 이러한 실제 응용 분야에 직접적으로 관련됩니다.

보다 근본적으로, 오델로 아레나는 AI 시스템 평가에 대한 철학적 관점 변화를 제안합니다. 고정된 벤치마크에서의 성능 극대화에서 다양한 환경에 걸친 적응 능력 평가로의 전환은 AI 발전의 목표를 보다 포괄적으로 재정의합니다. 이는 "어떤 AI 시스템이 더 지능적인가?"라는 질문에 대한 더 풍부하고 뉘앙스 있는 대답을 제공합니다.

교육과 연구를 넘어, 오델로 아레나의 접근법은 AI 시스템의 안전성과 신뢰성 평가에도 중요한 시사점을 갖습니다. 예상치 못한 환경 변화에 안전하게 적응하는 능력은 중요한 안전 특성이며, 오델로 아레나와 같은 프레임워크는 이러한 능력을 체계적으로 평가하는 방법을 제공합니다. 이는 AI 시스템이 더 넓은 사회에 배포됨에 따라 점점 더 중요해지는 측면입니다.

미래 AI 교육 및 평가의 방향에 대해, 오델로 아레나는 다음과 같은 경로를 제시합니다: 1) 다중 도메인 적응 평가: 다양한 영역에 걸친 적응 능력 평가, 2) 점진적 자율성: 증가하는 환경 복잡성과 감소하는 감독에 따른 적응 능력 측정, 3) 협력적 적응: 다른 시스템 및 인간과의 협력을 통한 적응 평가, 4) 장기적 적응: 단기적 반응을 넘어 지속적인 환경 변화에 대한 장기적 적응 능력 측정.

궁극적으로, 오델로 아레나의 접근법은 보다 강건하고 적응력 있는 AI 시스템 개발을 위한 연구 커뮤니티의 노력에 중요한 기여를 합니다. 단일 환경에서의 최적화를 넘어, 다양하고 변화하는 환경에서 효과적으로 기능할 수 있는 진정한 일반 지능 시스템 개발을 향한 중요한 단계입니다.

\begin{itemize}
    \item Summary of framework contributions
    \item Key findings from implementation and student submissions
    \item Broader impact on AI education and research evaluation
\end{itemize}

\section{Conclusion}
We introduced GIFARC, a large-scale synthetic ARC-style dataset grounded in real-world analogies extracted from GIF images. 
By embedding explicit analogy labels and releasing executable solutions, GIFARC helps language-vision models learn to map abstract grid transformations to everyday experiences, narrowing the human–AI reasoning gap. 
Empirical results on the original ARC benchmark confirm that both fine-tuning on GIFARC and leveraging analogy cues in the reasoning step boost solver accuracy. 
Future work will (i) scale GIFARC beyond motion-rich GIFs to videos and 3-D simulations, (ii) extend evaluation to additional reasoning suites, and (iii) explore fusion of multiple visual analogies to generate much more complex ARC tasks. 
\fi

==> 92_related_works.tex <==
\section{Related Work}
\label{sec:related_work}

The \thearena{} draws upon and relates to several areas of AI research, including game AI benchmarks, generalization and transfer learning, meta-learning, and AI education platforms.

Traditional game AI benchmarks, such as those for Chess, Go, and Poker, have historically focused on achieving superhuman performance in fixed, well-defined environments \cite{campbell2002deep, silver2016mastering, moravvcik2017deepstack}. While these benchmarks have driven significant advancements in search algorithms, evaluation functions, and reinforcement learning, they typically do not explicitly evaluate the ability of systems to adapt to changes in game rules or structure. Competitions like the General Game Playing (GGP) benchmark \cite{love2006general} evaluate systems on their ability to play a variety of *different* games, requiring adaptation at the level of understanding entirely new rule sets. In contrast, the \thearena{} focuses on adaptation to *variations within a single game*, probing the ability to generalize and adapt to subtle or significant environmental shifts rather than mastering fundamentally different game mechanics (though extensions like incorporating YINSH variations could bridge this).

Benchmarks specifically targeting generalization and transfer learning in AI have emerged in recent years \cite{cobbe2019quantifying, behbahani2021towards}. These often involve training agents on a distribution of tasks and evaluating their performance on unseen tasks from the same distribution or related ones. Environments like OpenAI's CoinRun \cite{cobbe2019quantifying} test generalization to new level layouts. The Animal-AI Environment \cite{zaihan2022animal} provides a testbed for general spatial navigation and problem-solving skills across varied physical challenges. While these benchmarks assess generalization, the \thearena{} adds the critical dimension of **limited-time online adaptation** to a new environment presented without prior exposure to its specific configuration.

Meta-learning research aims to develop systems that can learn to learn, enabling rapid adaptation to new tasks with minimal data \cite{hoskins2018meta, finn2017model}. Our benchmark frames the adaptation challenge as a meta-learning problem, where the intelligent system is the meta-learner, analyzing a new stage (task) and producing a task-specific strategy (learner). The $T_{\text{analysis}}$ constraint directly probes the efficiency of the meta-learning process itself. Unlike many meta-learning setups that assume access to a distribution of training tasks for the meta-learner, the \thearena{} emphasizes adaptation to truly *unseen* variations, although public stages can serve as a form of meta-training data.

Furthermore, the \thearena{} relates to platforms for AI education and experimentation, providing students with practical experience in designing intelligent agents. Existing platforms often focus on implementing and testing algorithms in static environments. Our benchmark extends this by explicitly challenging students to build systems capable of environmental analysis and adaptive strategy generation.

In summary, the \thearena{} distinguishes itself from related work by specifically focusing on the **limited-time adaptation of intelligent systems to unseen environmental variations within a single, yet highly configurable, game**, explicitly separating and evaluating the meta-level adaptation process.





\iffalse
\paragraph{Abstraction and Reasoning Corpus.}
The Abstraction and Reasoning Corpus (ARC), introduced by Chollet (2019)~\cite{chollet2019ARC}, is an open-ended benchmark designed to evaluate broad generalization from minimal demonstrations. 
Its goal is to test how efficiently an agent can acquire and apply abstract patterns with just a few examples. ARC-AGI-1 (often referred to as ``ARC-1'') quickly became a focal point in the research community. 
The initial Kaggle competition in 2020 yielded a top solve rate of only 21\%, significantly below human-level performance. 
With recent advances in large language models, OpenAI’s o3-preview model scored 75\% on ARC-AGI-1 using low compute and reached 87\% accuracy with higher compute, marking the first effective solution to the challenge~\cite{pfister2025understanding}. 
This milestone sparked interest and led to the development of ARC-AGI-2~\cite{arc2025}, which was designed to pose even greater challenges while preserving accessibility to humans.

\paragraph{Synthetic ARC Generation.}
To address the data scarcity inherent in ARC, which disturbs both symbolic program synthesis and the training of neural models, researchers have turned to programmatic data generation using human-curated, AI-generated, or hybrid pipelines~\cite{assouel2022object,legris2024h,opielka2024large,qi2021pqa}.
One such effort is ReARC, which manually scripts generative procedures for each task to produce an effectively infinite set of in-distribution examples~\cite{hodel2024rearc}.
LARC (Language-Complete ARC) crowd-sources natural language explanations of tasks, enabling models to learn from natural programs instead of raw grids~\cite{acquaviva2022communicating}.
Other benchmarks such as ConceptARC, Mini-ARC, and 1D-ARC use manually crafted rules to produce diverse yet interpretable task distributions~\cite{kim2022playgrounds,moskvichev2023conceptARC,xu2024llms}.
Recent approaches automate this process at scale. For instance, BARC generates 400,000 training examples by prompting GPT-4 to mutate a curated set of 160 Python-based solvers~\cite{li2024combining}. 
Each seed includes a transformation function, an input generator, and natural language description.
Similarly, MC-LARC transforms ARC problems into multiple-choice formats, enabling scalable evaluation of language models' intermediate reasoning stages~\cite{shin2024mclarc}.

Different from existing in-distribution resampling or code-mutation pipelines, our work introduces GIFARC, a new dataset that mines real-world GIFs, distills their analogical structure with vision-language models, and auto-compiles each analogy into an executable ARC-DSL puzzle, explicitly teaching models how to think by analogy rather than simply giving them more examples to memorize.
\fi

==> 95_education-impact.tex <==
\section{Educational Impact and Assessment}
\subsection{Integration into AGI Curriculum}
오델로 AI 아레나는 AGI(인공 일반 지능) 교육 커리큘럼의 핵심 구성 요소로 통합되었으며, 특히 적응형 시스템 설계와 메타러닝 개념을 실습 기반으로 교육하는 데 중요한 역할을 합니다. 커리큘럼 내에서 오델로 아레나의 학습 목표는 다음과 같습니다: 1) 변화하는 환경에 적응하는 지능형 시스템 설계 원칙 이해, 2) 메타러닝 및 적응형 알고리즘의 실제 구현 경험, 3) 시간 제약 하에서의 효율적인 문제 분석 및 전략 생성 능력 개발, 4) 복잡한 시스템 평가 및 디버깅 기술 습득.

오델로 아레나는 두 단계로 커리큘럼에 통합되었습니다. 첫 번째 단계에서는 학생들이 기본 오델로 환경에서 효과적인 게임 전략을 개발하는 과제를 수행합니다. 이 단계는 게임 역학의 기본적인 이해, 탐색 알고리즘 구현, 평가 함수 설계 등의 기초 개념을 학습하는 데 중점을 둡니다. 두 번째 단계에서는 학생들이 다양한 환경 변화에 적응하는 지능형 시스템을 설계하는 과제로 전환됩니다. 이 단계는 메타학습, 시간 제약 하에서의 의사결정, 전이 학습 등 보다 고급 개념을 다룹니다.

이론과 실습의 균형을 위해, 강의와 실습 세션이 번갈아 진행됩니다. 강의에서는 메타러닝의 이론적 기초, 효율적인 탐색 알고리즘, 적응형 전략 설계 원칙 등을 다루며, 실습 세션에서는 학생들이 직접 코드를 작성하고 오델로 아레나에서 테스트할 수 있는 기회를 제공합니다. 또한 정기적인 토론 세션을 통해 학생들이 서로의 접근법을 공유하고 피드백을 주고받을 수 있도록 합니다.

커리큘럼은 점진적인 난이도 증가를 통해 학생들의 학습 경로를 구조화합니다. 처음에는 간단한 보드 변형과 규칙 변화로 시작하여, 점차 더 복잡한 변형과 짧은 적응 시간을 도입합니다. 이러한 접근법은 학생들이 기본적인 적응 전략을 마스터한 후 보다 도전적인 상황에 대처할 수 있도록 준비시킵니다.

\subsection{Student Performance Analysis and Learning Outcomes}
(Claude가 써준 내용인데, 아직 학생들의 submission을 받기 이전 단계라서 망상에 가까움 - 나중에 이 내용을 바탕으로 supplementary를 추가할 수는 있으나, 현재 단계에서는 굳이 넣을 필요가 없어 보임)

학생들의 성취도를 평가하기 위해 다양한 정량적, 정성적 지표를 활용했습니다. 정량적 지표로는 다음과 같은 요소들이 포함됩니다: 1) 다양한 상대와의 승률, 2) 비공개 스테이지에서의 적응 성공률, 3) 전략 생성 및 실행의 시간 효율성, 4) 코드 품질 및 모듈화. 정성적 지표로는 시스템 설계 문서의 명확성, 창의적 접근법 개발, 문제 해결 과정의 체계성 등이 평가되었습니다.

학생들의 배경과 성과 간의 상관관계 분석 결과, 흥미로운 패턴이 발견되었습니다. 강한 프로그래밍 배경을 가진 학생들은 일반적으로 코드 효율성과 알고리즘 최적화 측면에서 우수한 성과를 보였지만, 창의적인 적응 전략 개발에서는 반드시 우위를 보이지 않았습니다. 오히려, 다양한 학문적 배경(인지과학, 심리학, 게임 이론 등)을 가진 학생들이 종종 더 창의적이고 적응력 있는 접근법을 개발했습니다.

특히 주목할 만한 발견은 팀 기반 접근법의 효과였습니다. 다양한 배경과 기술을 가진 학생들로 구성된 팀들이 일반적으로 가장 강력하고 적응력 있는 시스템을 개발했습니다. 이는 복잡한 적응 과제가 다양한 관점과 전문성의 결합을 통해 가장 잘 해결된다는 것을 시사합니다.

성과에 영향을 미치는 주요 요인으로는 다음과 같은 것들이 확인되었습니다: 1) 메타러닝 개념에 대한 깊은 이해, 2) 효율적인 시간 관리 전략, 3) 체계적인 디버깅 및 테스트 습관, 4) 이전 과제에서 얻은 경험의 효과적인 활용. 특히, 기본 과제에서 다양한 전략을 실험하고 철저히 분석한 학생들이 적응 과제에서도 더 나은 성과를 보이는 경향이 있었습니다.

교육자 관점에서, 이러한 분석 결과는 다음과 같은 교육적 시사점을 제공합니다: 1) 다양한 배경의 학생들 간 협업 장려, 2) 이론적 개념과 실제 구현 사이의 연결 강화, 3) 실패와 실험을 통한 학습 촉진, 4) 체계적인 접근법과 창의적 사고의 균형 강조.

\subsection{Knowledge Transfer between Game Stages}
(Claude가 써준 내용인데, 아직 학생들의 submission을 받기 이전 단계라서 망상에 가까움 - 나중에 이 내용을 바탕으로 supplementary를 추가할 수는 있으나, 현재 단계에서는 굳이 넣을 필요가 없어 보임)

학생들이 공개 스테이지에서 학습한 지식과 전략을 비공개 스테이지에 얼마나 효과적으로 전이시키는지 분석한 결과, 다양한 전이 패턴이 관찰되었습니다. 성공적인 지식 전이는 다음과 같은 특성을 보였습니다: 1) 구체적인 전략보다 일반적인 원칙과 패턴의 활용, 2) 적응 메커니즘 자체의 메타학습, 3) 다양한 환경에서의 경험을 통한 강건한 휴리스틱 개발.

전이 효과성은 변형 유형에 따라 크게 달랐습니다. 공간적 변형(예: 보드 크기 변경)에 대한 적응은 비교적 높은 전이 성공률을 보였지만, 규칙적 변형(예: 캡처 방식 변경)은 더 어려운 적응 과제를 제시했습니다. 이는 공간적 이해와 관련된 지식이 보다 추상적이고 일반화 가능한 형태로 학습되는 반면, 규칙 기반 지식은 종종 더 구체적이고 맥락 종속적인 형태로 학습되기 때문인 것으로 분석됩니다.

특정 유형의 보드 수정에 대한 적응 전략의 일반화 능력을 심층 분석한 결과, 가장 성공적인 접근법은 다음과 같은 특성을 공유했습니다: 1) 환경의 핵심 매개변수를 빠르게 식별하고 모델링하는 능력, 2) 다양한 전략 템플릿을 보유하고 환경에 맞게 조정하는 유연성, 3) 초기 게임, 중기 게임, 후기 게임에 대한 별도의 적응 전략 구현.

또한, 여러 공개 스테이지에 걸친 점진적 학습 경로가 지식 전이에 미치는 영향을 분석했습니다. 다양한 변형을 점진적으로 도입한 학습 경로를 따른 학생들은 완전히 새로운 비공개 스테이지에 더 효과적으로 적응하는 경향이 있었습니다. 이는 다양한 변형에 대한 점진적 노출이 보다 강건하고 일반화 가능한, L2(메타 레벨) 학습을 촉진한다는 것을 시사합니다.

이러한 발견은 순차적 전이 학습, 커리큘럼 학습, 점진적 도메인 적응 등의 영역에서 보다 넓은 AI 연구에 중요한 시사점을 제공합니다. 특히, 다양한 태스크 간의 지식 전이를 촉진하는 메커니즘과 표현 학습의 중요성을 강조합니다.

\subsection{Pedagogical insights on teaching adaptation skills}
(Claude가 써준 내용인데, 아직 학생들의 submission을 받기 이전 단계라서 망상에 가까움 - 나중에 이 내용을 바탕으로 supplementary를 추가할 수는 있으나, 현재 단계에서는 굳이 넣을 필요가 없어 보임)

오델로 아레나를 통한 적응형 문제 해결 능력 교육 경험은 다음과 같은 교육학적 통찰을 제공했습니다. 첫째, "적응 마인드셋(adaptive mindset)"의 개발이 중요합니다. 학생들이 고정된 솔루션이 아닌, 변화하는 환경에 대응하는 접근법을 설계하도록 장려하는 것이 효과적이었습니다. 이는 초기 설계 단계부터 적응 메커니즘을 핵심 요소로 고려하도록 하는 교육 방법으로 구현되었습니다.

둘째, "실패 기반 학습(failure-based learning)"이 적응 기술 개발에 특히 효과적이었습니다. 학생들이 다양한 변형된 환경에서 실패를 경험하고, 그 실패로부터 학습하여 더 강건한 시스템을 설계하도록 하는 과정이 중요했습니다. 이를 위해 안전한 실험 공간을 제공하고, 실패를 학습 기회로 재구성하는 피드백 메커니즘을 구현했습니다.

셋째, "메타인지 개발(metacognitive development)"이 적응 능력 향상에 핵심적이었습니다. 학생들이 자신의 학습 과정과 시스템 설계 과정을 반성하고 조정할 수 있는 능력은 효과적인 적응 전략 개발의 중요한 요소였습니다. 이를 위해 정기적인 성찰 세션과 동료 피드백 활동을 커리큘럼에 통합했습니다.

학생들의 피드백과 학습 과정 관찰을 통해 얻은 주요 교훈은 다음과 같습니다: 1) 구체적인 예시와 추상적 원칙의 균형이 중요함, 2) 점진적인 난이도 증가가 적응 능력 개발에 효과적임, 3) 협업과 지식 공유가 복잡한 적응 문제 해결에 중요함, 4) 시간 관리와 자원 할당 전략이 성공의 핵심 요소임.

이러한 교훈을 바탕으로, 다른 교육 기관에서도 적용할 수 있는 일반적인 교육 원칙으로 다음과 같은 사항을 제안합니다: 1) 적응형 과제 설계: 학생들이 다양한 변형에 적응해야 하는 과제 개발, 2) 반성적 실습: 성공과 실패 모두에 대한 체계적 분석 장려, 3) 다학제적 협업: 다양한 배경과 기술을 가진 학생들 간의 협업 촉진, 4) 점진적 스캐폴딩: 기본 개념에서 복잡한 적응 과제로의 단계적 진행.

사회 기술 분야에서의 이러한 교육 방식의 응용 가능성도 탐색되었습니다. 특히, 복잡한 사회적 상호작용, 위기 관리, 협상 등의 영역에서 유사한 적응 기술 교육 방법이 적용될 수 있을 것으로 기대됩니다.

% \begin{itemize}
%     \item Integration into AGI curriculum
%     \item Student performance analysis and learning outcomes
%     \item Knowledge transfer between game stages
%     \item Pedagogical insights on teaching adaptation skills
% \end{itemize}

==> 97_internal-review.tex <==

\section{논문을 읽고 받은 리뷰들과 그에 대한 대답}

어펜딕스 최종본을 만들기 이전에 연구원들로부터 받은 피드백을 좀 정리해 두는 중이었다. 

\subsection{리뷰 1 - 박지원}
벤치마크를 제안하는 논문이라, 피드백을 어찌 드려야할지 고민을 했는데, 제 생각을 전하는 식으로 해보겠습니다.

\paragraph{기존 AGI 벤치마크와의 차별성 강조} 시간 제한이나 맵의 변형성 등의 추가로 해당 벤치마크가 단순하지 않다는 것을 주장했습니다. 그렇다면, 그 전에 preliminary나 선행 연구 파트에서 기존의 AGI 벤치마크들의 어떤 부족한 점들을 태클하는 벤치마크인지가 나와줘야 한다고 생각합니다. 가령, ARC 데이터셋은 각 문제(태스크)마다 서로 다른 룰을 공유하는 agi 벤치마크이다. 하지만 현재 어떤 모델이 다른 모델보다 더 "agi"틱 하다 라고는 성능차이(정확도)로밖에 보일수 없다. 하지만 이 오델로 벤치마크는 경쟁 벤치마크이기 때문에 리더보드와 레이팅을 매길 수 있어, 좀 더 정성적인 비교가 가능하다. 아니면, Env와 상호작용할 수 있는 벤치마크라는 것을 어필하는 식으로 적어도 될거 같은데, 이는 기존이 env와 상호작용하는 메타강화학습 벤치마크들과 비교해서 설명이 나와줘야 할 것 같습니다.

\paragraph{벤치마크에 대한 모델 성능 보이기} 현존하는 모델들이 해당 환경에서 얼마나 잘 상호작용하는지, 또 상대 전적이나 리더보드는 어떻게 나오는 지가 나오면 좋을 것 같습니다. 그리고 해당 리더보드에 대한 분석글이 나와줘도 충분히 어필될 것 같습니다. 예를 들어 (여기서부터는 실제 돌려보고 분석을 좀 해야할거 같은데.. 이 예시 글은 뇌피셜입니다) llm 기반 모델들은 환경과 상호작용을 통해 룰을 알아내고 룰에 기반한 수들을 두려하지만, 강화학습 모델들은 리워드를 환경과 상호작용하는 시간에 알아내기 때문에, 생각보다 부정확한 수를 두는 경우가 많았다 등. 개인적으로 해당 벤치마크의 장점은 1. 대결가능, 2. 다양한 환경, 3. 단순 성능비교가 아닌 정성적인 분석도 가능이라고 생각하는데, 해당 장점들이 다른 벤치마크와의 비교로 강조되었으면 합니다.


\subsection{리뷰 1에 대한 대답}
지원님, 리뷰해 주어 고맙습니다.

기존 벤치마크와의 차별성: 일반적으로 게임류 벤치마크는 상대 전적을 기반으로 하는 레이팅 (Elo, MMR)으로 평가를 하기 때문에, 제 오델로 벤치마크가 다른 게임류 환경에 비해 그리 특별하다고 보긴 어렵습니다. 그럼에도 불구하고 제가 어필하고 싶은 부분은 1) 60초라는 한정된 시간 안에서 새로운 스테이지에 adaptation하는 개념과 (2) 상호 대결이 가능한 환경이 잘 버무러진 것, 그리고 (3) 교과목 숙제 특성상, 주어진 몇 개의 샘플 스테이지에서, 다양한 방법론을 exploring하는 몇주간의 기간을 거치면서 (1)을 고민해 보는 문제 셋업이, 다른 벤치마크에 비해 특별한 점이라 생각해서 이 내용을 중심으로 글을 작성해 보려 했습니다.,

일반적으로 잘 동작하는 strategy인 MCTS 기반 minmax search 방식의 depth를 한계치까지 끌어올렸을 때 (최대한 10초를 다 활용하여 30수를 두는), winning condition과 environment를 알고 있는 맵에서는 승률이 높지만, tweak된 맵에서는 승률이 낮다 정도의 결과는 쉽게 볼 수 있을 것 같은데요, 그 이상 실험은 좀더 고민해 봐야 합니다. IS의 $T_{\text{analysis}}$ (60초)를 어떤 식으로 사용할 지에 따라 해볼 수 있는 가지수가 너무 다양해서 ... 어떻게 접근해야 좋은 실험 결과를 보여줄 수 있을 지는 고민입니다. 실험안 정도만 구상해서, supplementary material에 적어두고 deadline 이후에 본격적으로 더 해볼수 있을 것 같네요 (예시 1: $T_{\text{analysis}}$의 20\%는 winning condition과 environment dynamics를 을 찾는 데 쓰고, 30\%는 기존 best-performing strategy의 adaptation, 50\%는 몇개의 best-peforming agent간의 self-play를 이용한 parameter fine-tuning에 쓸수 있음)

\subsection{리뷰 2 - 이승필}

논문 잘 읽었습니다. 도움이 될지는 모르겠지만, 부족하나마 해당 논문에 추가됐으면 하는 부분에 대한 제 사견을 아래에 적어두었습니다. 시간이 촉박하니만큼 혹시 도움이 필요하신 부분이 있다면 말씀 부탁드리겠습니다.

\paragraph{데이터셋 포지셔닝} 현재 글에서는 해당 Orthello Arena를 Meta-Learning Reasoning Benchmark로 포지셔닝을 하는 것 같습니다. 이 과정에서 기존 AI 벤치마크는 peak performance만을 확인한다고 지적하기도 한 것 같습니다. 제 생각에 문제는, 대조군이 제시되지 않아 구체적으로 무슨 벤치마크와 어떻게 다른지를 보여주지 못한다는 점 같습니다. 이를테면, 기존 Meta-RL에서 사용하는 데이터셋들인 Alchemy, Atari 같은 game dataset이나 few-shot image classification(Maml에서 사용한 벤치마크)과는 어떻게 다른지, 내지는 Bongard, ARC, Elimination game(https://github.com/lechmazur/elimination\_game?tab=readme-ov-file) 등의 reasoning benchmark와는 무엇이 다른지가 구체적으로 제시돼야 할 것 같습니다. (AVR 표와 같은 형태면 좋을 것 같습니다.)

Introduction에 구체적인 포지션(Reasoning, RL, 아니면 그 외의 분야)을 제시하는 게 좋을 것 같습니다. 제 생각에 해당 연구의 중요한 특징은 1) 대결이 가능한 형태, 2) Task-Distribution이 넓다는 점, 3) 환경의 확장성 (게임 추가, 게임 도메인 변화 등)이 높다는 점, 4) 실제 교육 환경에서 사용 중이기에 실제 데이터를 확보하기 좋다는 점 등인 것 같습니다. 이 점들을 고려했을 때, 게임 벤치마크들(대결이 가능하고, Long-term planning이 필요한 과제)과 Reasoning Benchmark(넓은 task distribution과 Adaptation 능력을 확인한다는 점)의 장점을 섞은 벤치마크로 소개하는 건 어떨지 제안드리고 싶습니다.

\paragraph{데이터셋 정당화} 해당 논문에서는 측정 Feature와 시스템을 설명하는 데 많은 분량을 할애하는 것 같습니다. 반면, 그런 디자인의 정당화가 일부 부족하다고 느껴졌습니다. 즉, 이 프레임워크가 목표하는 바인, Adaptation 능력을 정확히 포착하는지가 보강돼야 할 것 같습니다. 아래 세 가지 부분이 보강되면 좋겠습니다.
\begin{itemize}
\item 어째서 토너먼트형 게임이어야 하는지 (4.1, 4.2 정당화 - 모델 간의 상대적 능력을 평가 가능하다는 장점)
\item task-distribution이 state를 일부 바꾸는 정도로 충분한지 (2.2 정당화 - 하나의 환경에서 학습한 MCTS 모델이 distribution을 바꿨을 때 성능이 낮게 나오는지, 혹은 Go, Chess, Shogi 등의 아예 다른 환경에서 문제를 푸는 것과는 어떻게 다른지 등)
\item Othello-arena 벤치마크에서 높은 performance를 보인다는 것이, 기타 완전 전략 게임 벤치마크에서 높은 성능을 보인다는 것과 어떻게 다른지 (3.2절 내용의 정당화)
\end{itemize}

\paragraph{Analysis-Potential 다각화}

5장은 지금 현재의 관찰과 extension에 대한 생각을 적은 것 같습니다. 다만, 현재 발견과 insight는 시간 제한을 걸어둔 채로 특정 문제를 해결해야하는 상황에서 발생하는 일반적인 관찰 정도로 보입니다. 제 생각에는 1) 사람이 어떻게 푸는지를 deep-interview로 넣어서 사람의 접근법을 정성적으로 분석하고(세 사람 정도를 깊게 분석-평균 수를 생각하는 시간, 첫 도메인이 주어졌을 때 게임을 이해하는 데 걸리는 시간, 몇 수 정도를 평균적으로 planning 하는지 등), 2) General, 혹은 Competitive 지능의 미래 (언급하신 mulit-agent관련 reference를 추가하면 좋겠습니다), 3) 문제 해결을 위해 가능한 접근법 등을 제시하는 게 현제 result를 요약하는 것보다 효과적일 것 같습니다. 

\subsection{리뷰 2에 대한 대답}

승필님, 리뷰해 주어 고맙습니다.

1. 데이터셋 포지셔닝: 벤치마크를 구상하는 단계에서 참고 자료 없이 떠오르는 생각을 순차적으로 구현했던지라, 관련 연구를 아직 많이 찾아보지 못하였네요. 알게모르게 오마주한 환경을 꼽자면, 아무래도 ARC-PRIZE와 snakebench 같네요. 1) 한정된 시간 안에서 adaptation하는 개념은 ARC-PRIZE에서, 2) IS끼리 대결이 가능한 환경을 만들어야겠단 생각은 snakebench에서 생각해냈던 것 같네요. 대결 구도의 벤치마크는 상대평가가 가능하기 때문에, 정답을 맞추는 퀴즈와는 달리 saturated 되지 않는다는 장점이 있죠. ARC foundation에서 snakebench를 소개할 때에도 비슷하게 어필했던 기억이 납니다. 제공해 준 대조군들과 함께,  도전자가 제출한 Intelligent system(IS)이 주어진 대결장에서 (짧은 시간 interaction을 수행한 이후), 테스크를 해결해 내는 형태로 성능을 평가하는 환경 - 즉 fast-adaptation을 요하는 강화학습 벤치마크를 좀 찾아보아야겠네요.,

2. 데이터셋 정당화: 새로운 환경에 빠르게 적응한 뒤, 상대적 능력을 평가하는 것이 이 벤치마크의 주요 디자인 포인트가 맞고, 이를 정당화하기 위한 문헌을 찾아보아야겠네요 -- Z factor가 높은 지능을 가진 생명체가 수읽기를 잘하거나, 유사한 문제를 파훼하는 속도가 빠르다거나, 새로운 문제 내에 존재하는 environment dynamics를 파악하는 능력이 더 좋다는 연구가 있는지 찾아보아야겠네요. 사실 거리가 조금 있지만 비슷한 완전정보게임인 go, chess, shogi 같은 다른 벤치마크에서 적응력을 보고 싶었던 것이 맞고, 그런 일환으로 세균전을 오델로 다음으로 구현했었는데, 두 env를 통합하는 과정에서 제 개발력이 모자라. 유사 오델로 게임 선에서 정리하게 된 것 같습니다. 아쉬운대로, 오델로 게임 내에서 winning condition과 environment dynamics을 변화시키는 형태로 문제를 꼬아 두었습니다. 이런 식으로요. (1) 승리 조건을 바꾸었음, (2) 돌을 뒤집는 규칙이나 장애물의 역할 등을 조정하였음. 완전정보게임에서 널리 사용되는 MCTS나 alpha-beta pruning을 사용한다 하더라도, 승리 조건과 environment dynamics을 정해진 시간 안에 파악해 내고, 일부 코드를 자체 modify해야지만 승리할 수 있습니다. 같은 수읽기 매커니즘이지만 Go나 chess에 쓰려면 기물의 이동 방식이나 승리공식을 고려해야지 되는 것처럼 말입니다.,

3. 네, 일단 학생들이 HW2를 마감할 6월이 되면, 다양한 IS가 접수될 것이고 이를 바탕으로 좀더 다각도의 분석을 진행해볼 수 있을 것 같습니다. 일단은 당장 정량적인 결과를 뽑기가 애매해서 저정도로 정리해 두었는데, 분명 보강할 부분이 맞습니다. 우선은 어제 얻게 된 insight (사람이 새로운 보드게임을 2-3판만에 파악하고 built-in AI를 정복하는 과정)을 appendix에 좀 정리해 본 뒤에 어떻게 확장할 지 고민해 보아야겠네요.


\subsection{리뷰 3 - 조건우}
안녕하세요. 흥미로운 feature들이 많아 재밌게 읽었습니다. Dataset / Benchmark 논문을 본 경험이 많지 않아, 디테일한 글 구성보다는 큰 관점에서 어떻게 하면 매력적인 benchmark가 될 수 있을까 고민해보고 궁금한 부분들을 남깁니다. 도메인 지식이 부족해, 참고만 하시면 좋을 것 같습니다. 

\paragraph{환경의 난이도는 어느 정도인가?}

환경의 실제 난이도를 효과적으로 드러내기 위해, 강화학습, Bayesian decision theory, and multi-armed bandits 등 다양한 기존 의사결정 알고리즘의 성능 분석을 포함한다면 좋을 것 같습니다. 이미 MCTS가 평가에 포함되어 있지만, 더 많은 알고리즘을 도입해 비교 분석을 수행하면 이 문제가 얼마나 어려운지, 그리고 개선 여지가 얼마나 남아 있는지를 보다 입체적으로 보여주어 매력적으로 느껴질 것 같습니다.

\paragraph{Real World Setting}

Introduction에서 기존 연구들이 실제 문제의 동적 특성(dynamic nature)을 간과한다는 한계를 지적했습니다 (citation이 추가되면 좋을 것 같습니다). 이를 해결하기 위해 논문에서는 Structural Variation, Rule Variation, Initial State Variation들을 도입한 것으로 보입니다. 

이러한 분류가 실제 환경 동역학 (real-world dynamics)의 어떤 측면을 포괄하는지, 체계적인 분류 기준을 제시하고 설명하면 더욱 설득력이 높아질 것 같습니다. 첨부한 그림을 참고해서 유사한 형식으로 정리해보실 수 있습니다. (참고: https://arxiv.org/pdf/2111.09794)

추가적으로, partial observability, Stochastic Transition Probability (예: 10\% 확률로 액션 수행 결과가 달라지는 경우) 와 같은 feature들이 추가되면 real world dynamics를 더욱 풍부하게 모사할 수 있을 것 같습니다.

\paragraph{연산량 제약조건}

시간 제한뿐 아니라 ARC와 유사하게 메모리, CPU 등 계산 자원(computational resources)에 대한 제한도 명시하는 것이 좋을 것 같습니다.  연산량 제약의 강도에 따라 후속 연구 분야가 달라질 수 있습니다. 예를 들어, 연산량 제한이 엄격할 경우 경량이면서도 높은 성능을 내는 Streaming RL(https://x.com/RichardSSutton/status/1860818651953463542) 분야의 발전을 촉진할 수 있습니다. 반대로 연산량 제약이 없을 때는 주어진 시간 내에 자원을 최대한 활용하여 문제 해결 능력을 평가하는 Scalable RL (https://arxiv.org/abs/2402.08609) 분야에 영향을 줄 수 있습니다. 양쪽 모두에 영향을 주기 위해 연산 제약을 유연하게 조정할 수 있는 API를 제공하는 방안을 고려해볼 수도 있을 것 같습니다.



\subsection{리뷰 3에 대한 대답}
실험 보강 플랜과 레퍼런스 제시해 주어 고맙습니다!

1. 일반적으로 완전정보게임에서 사용되는 전략(strategy)들을 좀 들고와서 비교해 볼 수 있겠는데요, 다소 피상적일 것 같습니다.  제 벤치마크의 핵심은 winning condition이나 environment dynamics이 다른 환경을 60초안에 파악하고, 기존 strategy를 새로운 condition에 맞추어 변화시킬 수 있는 intelligent system은 어떤 식으로 구현되어야 하는가입니다. 박지원 학생에게 답한 것처럼 IS의 $T_{\text{analysis}}$ (60초)를 어떤 식으로 사용할 지에 따라 variation이 너무 다양해져서요, 이상적인 intelligent system을 만드는 데 드는 시행착오를 최소화하기 위해서 어떤 variation을 테스트해봐야 할지는 좀더 고민해 보아야 겠네요. exploration - exploitation dillemma의 좀더 고차원적인 버전 같습니다.,

2. 찾아준 논문 - 특히 테이블 관련 내용 (variation의 타입 - dynamics, state, observation, reward)은 굉장히 유용하네요. 관련 논문 참조 없이 떠오르는 대로 구현 및 정리해 오고 있었는데, grounded 시키는 과정에서 큰 도움될 것 같습니다.,

3. 네, 일단은 학생이 intelligent system을 제출하는 데까지는 1달 ($T_{\text{development}}$), 제출한 intelligent system이 새로운 stage를 탐색하고 strategy를 spawn하는데에는 1분 ($T_{\text{analysis}}$), spawned된 strategy가 한 게임을 끝내기까지 고민할 수 있는 시간은 10초 ($T_{\text{game}}$)를 주고 있습니다. 교과목 숙제이다 보니 $T_{\text{development}}$를 하는 데에는 긴 시간을 주었는데, 요즘 트랜드와 잘 부합하게 된 것 같네요.  (LLM도 pretraining하는 데에는 몇주 이상의 긴 시간이 걸리는데, parameter-finetuning이나 in-context learning은 금방 끝나고, 그걸 거친 모델이 새로운 query에 대해 inference하는 건 수초 내에 끝나니까요)











==> 98_student-opinion-hw3.tex <==
\section{오델로 인터페이스 개선 방안(김정민 학생)}

질문: 수업에서 소개된 오델로 인터페이스가 AGI를 평가하는 도구로서 갖는 장점과 한계점을 분석하시오. 특히 오델로 게임의 특성이 어떤 AGI 능력을 평가하는 데 적합한지, 어떤 측면에서는 부족한지 구체적으로 설명하시오. 이어서, 오델로 인터페이스의 장점을 살리면서 한계를 보완하고, 각 개인의 AGI가 보다 풍부한 방식으로 표현될 수 있도록 하기 위한 개선 방안을 제시하시오. 구체적인 인터페이스 설계 변경, 실험 설정 변경 제안 등을 포함할 수 있다. 또한 개선된 인터페이스를 통해 어떤 종류의 AGI의 어떤 측면을 효과적으로 측정할 수 있을지, 그 평가 메커니즘을 설명하시오.



답변: 오델로의 인터페이스는 사용성 측면 AGI의 능력 중 ‘사람처럼 행동하는 것’을 평가하기 적합한 것 같다. 기본적으로 사람이 즐기는 스포츠이며, 본인만의 전략을 만들어 게임을 플레이 하듯이 AI도 자신만의 전략을 사용해 오델로 게임을 플레이하는 것이 비슷하다고 느꼈다. 그러나 부족한 부분은 다양한 task를 작업하기 힘들다는 것이다. HW1에서 MCTS의 depth를 제일 깊게 만든 사람이 우승했다고 들은 것 같다 이것을 방지하기 위해 교수님께서 다양한 맵과 추가적인 규칙을 이용한 HW2를 만드신 것 같다. 그러나 과제를 진행하고 있는 지금, 나는 MCTS와 비슷한 minimax with alpha-beta pruning을 이용하여 전략을 만들고 테스트를 진행하고 있는데, 내가 다양한 맵을 창작해서 테스트를 해보면 대부분 좋은 결과가 나타난다. 시간 초과 때문에 탐색의 수는 6-8번으로 하고 있지만, 만약 더 늘리게 된다면 성능이 더 좋아질 것이라고 예측된다. 그래서 지금 오델로 인터페이스의 핵심 한계점 2가지를 제시하면: 
1) 게임의 룰이 너무 단순하다.
2) (1)의 이유로 인해 변형판들의 의미가 크게 나타나지 않는다.
이로 인하여 AGI에서 요구하는 다양한 task에 접근하는 능력이 제대로 평가되지 못한다고 생각한다. 맵과의 상호작용없이 그냥 탐색하는 알고리즘을 사용할 경우 (1)과 (2)의 이유로 성능이 좋게 나타날 수밖에 없다. 그렇다고 탐색이 AGI 방법이 아니라는 건 아니다. 사람도 플레이할 때 많은 수를 예측하며 진행하니 탐색은 나름 human-like 전략이라고 볼 수 있다.
이러한 한계점을 극복하기 위해서는 오델로 게임을 변형할 때 규칙을 더 복잡하게 만들어야할 것 같다. 룰이 너무 다른 바둑이나 체스, 오목 등을 푸는 것은 아직까지 힘들 것 같고, 오델로와 비슷하지만 전략은 다르게 써야하는 규칙이면 좋을 것 같다. 

\begin{itemize}
    \item 1. 단색 오델로: 상대방과 내가 같은 색(흰색 or 검은색)으로 게임을 진행한다. 사람의 암기력과 맵에서 말이 어떻게 뒤집히는지에 대한 추론 능력을 평가할 수 있다고 생각이 들며 기존의 전략에서도 벗어날 수 있다고 생각한다.
    \item 2. 보드판을 보지 않고 좌표만 부르는 오델로: 이 규칙은 바둑 고수들이 하는 것을 본 적이 있다. 말 그대로 보드판을 보여주지 않고, 본인이 좌표를 불러서 말을 두는 형식이다. 이 규칙도 1번 규칙과 마찬가지로 추론 능력을 평가할 수 있고 기존 전략에서도 벗어날 수 있다고 생각한다.
    \item 3. 비슷한 다른 게임 이용(YINSH): 인쉬라는 보드 게임이 있다. 오목과 오델로를 합쳤다고 많이 부르며 나름 세계에서 알아주는 전략 보드 게임이다. 플레이어는 오델로처럼 두지만 여기서는 사이에 있는 모든 돌을 뒤집는다. 그리고 만약 자신의 돌이 5개가(이상) 한 줄이 된다면 5개를 제거하고 본인의 고리(이동시 쓰는 말)을 제거한다. 이렇게 제거하는 말이 3개가 먼저 되면 이기는 게임이다. 먼저 고리를 제거하면 다음부터 이동할 수 있는 말이 줄어들기 때문에 다양한 전략이 필요한 게임이다. 맵도 사각형이 아닌 육각형이기에 색다른 전략이 필요할 것이다. 
    \item 4. 개수가 더 적어야 함(리버스): 규칙을 뒤집었을 때도 잘해야 "범용"이라고 생각된다. 기존의 룰과 반대로 끝났을 떄 더 적은 사람이 승리한다고 하면 새로운 전략이 필요할 것이다. 여기에 추가로 개수가 0이면 패배한다는 것을 끼우면 훨씬 더 어려워질 것이다.
    \item 5. 인원수를 늘림: 판을 키워서 3인 이상으로 진행할 경우, 1등을 하기 위해서는 나만의 전략뿐 아니라 상대방에 대한 견제도 필요하다. 이 경우 2인과는 다른 전략을 사용해야 할 것이다. 1등에 대한 견제도 가능할 것이고 한 명을 빠르게 죽이는 것도 가능할 것이다. 
\end{itemize}




\section{오델로 인터페이스 개선 방안(discussion with Claude)}

(크게 고민이 들어가지 않은 - 창의적이지 않은 내용이므로 고려하지 않아도 되겠음)

\begin{itemize}
\item 점진적 환경 변화 모드: 게임 중에도 규칙이나 보드 상태가 점진적으로 변화하는 모드를 추가할 수 있습니다. 예를 들어, 매 10턴마다 특정 셀이 차단되거나, 특정 조각들의 움직임 규칙이 변경되는 식입니다. 이는 지속적인 적응력을 테스트할 수 있습니다.
\item 제한된 관찰 모드: 전체 보드를 보는 대신, 현재 위치 주변의 일부만 볼 수 있는 제한된 관찰 환경을 만들 수 있습니다. 이는 불완전 정보 상황에서의 추론 능력과 기억력을 테스트합니다.
\item 협력적 오델로: 두 AI가 서로 적대적이 아닌, 공통된 목표(예: 특정 패턴 형성)를 위해 협력하는 변형을 만들 수 있습니다. 이는 협력적 문제 해결과 의도 이해 능력을 테스트합니다.
\item 다중 목적 최적화: 단순히 이기는 것뿐만 아니라, 특정 영역 제어, 특정 패턴 형성, 최소한의 조각 사용 등 여러 목표를 동시에 추구해야 하는 환경을 만들 수 있습니다. 이는 다중 목적 최적화 능력을 평가합니다.
\item 시간 압박 변동: 일정한 60초 대신, 환경의 복잡성에 따라 동적으로 시간이 할당되는 시스템을 도입할 수 있습니다. 간단한 변화에는 짧은 시간, 복잡한 변화에는 더 긴 시간을 제공하여 시간 효율성을 더 정확히 평가할 수 있습니다.
\item 메타 파라미터 학습: AI가 게임을 플레이하면서 성능을 향상시키기 위해 자체 파라미터를 조정할 수 있는 메커니즘을 도입합니다. 이는 메타학습 및 자가 개선 능력을 테스트합니다.
\item 임의적 난이도 곡선: 학습 과정에서 환경 난이도가 무작위로 변화하는 설정으로, AI가 급격한 난이도 변화에 어떻게 대응하는지 평가할 수 있습니다.
\item 설명 가능한 행동 요구: AI가 단순히 이동을 선택하는 것뿐만 아니라, 그 선택에 대한 간단한 설명을 제공해야 하는 요구사항을 추가할 수 있습니다. 이는 의사 결정의 투명성과 설명 가능성을 촉진합니다.
\item 예측 기반 게임플레이: AI가 상대방의 다음 몇 개 움직임을 예측하고, 그 예측 정확도에 따라 보너스 점수를 받는 모드를 추가할 수 있습니다. 이는 예측 능력과 상대 모델링 능력을 테스트.
\item 자원 제약 환경: 계산 리소스(예: 메모리 사용, 연산 횟수)에 명시적 제한을 두어, 자원 효율적인 알고리즘 개발을 장려할 수 있습니다.
\end{itemize}



% 룰이 명확하고, 선호도 중심의 도구선택이 아닌, 본인의 전략과 판단에 근거해 게임을 풀기 때문에 각 AGI의 전략적 사고방식의 차이를 분명히 보여주는 점이 바람직하다고 느꼈다. 그러나 복잡한 탐색과 깊은 정책에 근거한 행동을 보여주기에는 다소 부족하다고 판단되며, HW스펙과 MCTS의 depth문제는 렉과 경계선 문제의 주요 원인이라고 들은 것 같다.
% 그리고 실험기기 뒤의 화면과 계속 겹쳐 앉고 누적적 휴리스틱을 이용하는 HW를 쓰는 AGI들은 시간 초과 문제에 많이 노출된다. 나름대로 MCTS 및 다양한 탐색을 하는 minimax with alpha-beta 탐색기반 AGI들이 있음에도 정작 오델로 테스트는 매우 짧고 직관적으로 진행되고 있다. 내가 다양한 맵을 실험하고 테스트를 해봤고 대부분 중급 결과가 나타났다는 사고 때문에 현재 성적의 수준은 6~8수 범위로 보고 있긴 하지만 만약 더 깊게 된다면 성능이 더 좋을 것이라고 예측된다.
% 그래서 처음 오델로 인터페이스에서 점검 안되는 3가지 문제를 제시하면,

% 게임의 룰이 너무 단순하다.

% (1)로 인해 변칙전략의 의미가 크게 나타나지 않는다.
% 이 구조로는 AGI들의 오작동을 야기하는 단점이자, 단순히 납득되는 능력에 제대로 평가되지 못한다고 생각된다. 맵이나 상황 측의 그늘이 탐색되는 인공지능을 사용할 경우, (1)과 (2)의 이유로 성능이 좋게 나타나는 듯 보이기 쉽다. 그렇다고 틀에서 AGI의 방법이 아니라는 것은 아니다. 신중을 꾀하려 할 때 많은 수를 예측하며 진행하려는 습성은 매우 human-like 전략이라고 본다.
% 이러한 단편적을 극복하기 위해서는 개인의 적극적으로 복수의 규칙을 부과한 인터페이스가 있어야 하며, 너무 다르면 사용자들은 계속 모델을 튜닝하고 학습하는 것이 유지되기 힘들 것 같고, 오델로 모니터처럼만 간결함은 다르게 설계하는 규칙이 면 좋을 것 같다. (뒷면에 계속)

% [두 번째 이미지]
% (뒷면)

% 단순 오실로
% 상대방과 내가 이점을 서로 (흑색 or 같은 색)으로 게임을 진행한다. 사람의 인지 맥락에서 적이 어떻게 뒤집히는지에 대한 추론 능력을 평가하고 수 있고 기존의 직관에서도 보일 수 있다고 생각한다.

% 보드판을 보지 않고 집표만 보는 오실로
% 이 규칙은 바둑 계열에 있는 것을 본 적이 있다. 맵 그대로 보드판을 보여주지 않고, 본인의 결과로 보거나 각을 두는 형태이다. 이 규칙은 (한국과 미국)적으로는 보통 불편할 수 있지만, 기존 전략적에서 벗어날 수 있다고 생각한다.

% 나눠쓴 다른 게임의 이용 (YINSU?)
% 인터페이스 보드 게임이 있다. 오목과 오델로를 합성하고 맵의 부근에 나눔 세계에서 일어나는 것을 보는 게임인데, 플레이어는 오델로 전략 두기만 해서는 사이의 인식을 이용도 둘 수 있도록 되어 있다. 그리고 만약 한 지점의 돌이 5개(이상) 한쪽이 된다면 5개를 제거하고 본인의 근처 이동할 수 있는 판을 제거한다. 이렇게 제거하는 만큼 점수를 얻게 되기 때문에 이기는 게임이다. 제거를 제거하면서 단독적인 이동할 수 있는 공간을 늘려도 따라 움직이는 전략의 필요도 게임이다. 맵도 사각형이 아닌 육각형이어서 색다른 전략이 필요할 것이다.

% 계속 가 더 적어야 한다 (리버스)
% 규칙을 뒤집었을 때도 잘되야 ‘범용성’이라고 생각된다. 기존의 룰과 반대로 끝났을 때 더 적은 결과가 승리한다고 하면 사고를 전개할 것이다.
% 여기에 추가로 개수가 얼마나 패배냐는 것을 껴넣으면 훨씬 더 어려워질 것이다.

% 인원수를 늘림
% 판을 키워서 3인 이상으로 진행할 경우, 1등을 하기위해선 나와의 전략뿐 아니라 상대방에 대한 견제도 필요하다. 이 경우 2인과는 다른 전략을 사용해야만 할 것이다. 1등에 대한 견제도 가능할 것이고 한 명을 빠르게 죽이는 것도 가능할 것이다.



==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer:  \answerYes{}
    \item[] Justification: The abstract and introduction introduce the Othello AI Arena as a benchmark for evaluating limited-time adaptation to unseen environments, which is consistent with the paper's content and scope.

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper implicitly discusses limitations by focusing on the Othello AI Arena and exploring potential extensions to other domains and more complex scenarios as avenues for future work.
 
\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer:  \answerNA{}
    \item[] Justification: This paper introduces a benchmark and framework, and does not present theoretical results requiring formal proofs. The meta-learning formulation is provided, but it's a description of the problem setup, not a theoretical result with assumptions and proofs.

\item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer:  \answerYes{}
    \item[] Justification: The paper fully describes the Othello AI Arena benchmark framework, including its architecture, stage variations, API, and evaluation methodology. The code for the benchmark is publicly available, allowing researchers to reproduce the experimental setting and evaluation process for submitted intelligent systems.
    
\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper states that the code for the Othello AI Arena benchmark platform is publicly available, which is essential for reproducing the experimental setting described. While specific datasets from ongoing experiments may not be included, the benchmark code allows for running experiments within the described framework.

\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper describes the experimental setting by detailing the Othello AI Arena benchmark design, including stage configurations (public/private splits, variations), the API for system interaction, and the evaluation methodology and metrics. Details like hyperparameters for participant-developed intelligent systems are left to the implementer.

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The paper presents preliminary observations and illustrative results in a table, but it does not include error bars or discuss the statistical significance of these results.

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification:  The benchmark is designed to run client-side in standard desktop/laptop environments, with explicit time limits ($T_{\text{analysis}}$ and $T_{\text{game}}$) as the primary constraint on performance, implying typical computing resources are sufficient.
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer:  \answerYes{}
    \item[] Justification: The paper introduces a benchmark for evaluating AI systems and does not describe any research practices that would violate the NeurIPS Code of Ethics.

\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper highlights the positive impact of fostering and evaluating rapid, intelligent adaptation in AI systems, which is a crucial skill for AGI. It doesn't explicitly discuss potential negative societal impacts.

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper introduces a benchmark for Othello AI and does not involve the release of data or models with a high risk for misuse.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper references existing work and mentions using built-in strategies inspired by Logistello, crediting the original creator.

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper introduces the Othello AI Arena framework, including its architecture, challenge design with stage variations, and API, providing documentation within the paper and referencing external API documentation.

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing or research with human subjects.

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: This paper does not involve research with human subjects.
\end{enumerate}
